HiP-AD: Hierarchical and Multi-Granularity Planning with Deformable Attention for Autonomous Driving in a Single Decoder

Although end-to-end autonomous driving (E2E-AD) technologies have made significant progress in recent years, there remains an unsatisfactory performance on closed-loop evaluation. The potential of leveraging planning in query design and interaction has not yet been fully explored. In this paper, we introduce a multi-granularity planning query representation that integrates heterogeneous waypoints, including spatial, temporal, and driving-style waypoints across various sampling patterns. It provides additional supervision for trajectory prediction, enhancing precise closed-loop control for the ego vehicle. Additionally, we explicitly utilize the geometric properties of planning trajectories to effectively retrieve relevant image features based on physical locations using deformable attention. By combining these strategies, we propose a novel end-to-end autonomous driving framework, termed HiP-AD, which simultaneously performs perception, prediction, and planning within a unified decoder. HiP-AD enables comprehensive interaction by allowing planning queries to iteratively interact with perception queries in the BEV space while dynamically extracting image features from perspective views. Experiments demonstrate that HiP-AD outperforms all existing end-to-end autonomous driving methods on the closed-loop benchmark Bench2Drive and achieves competitive performance on the real-world dataset nuScenes.

==> table/supp_granularity.tex <==
\begin{table}[tb]\footnotesize
\centering
\resizebox{0.75\linewidth}{!}
{
\begin{tabular}{l|c}
\toprule
Multi-granularity       & Sampling Strategy  \\        
\midrule
Temporal waypoints      & 2m, 5m   \\
Spatial waypoints       & 2Hz, 5Hz \\
Driving-style waypoints & 2Hz $\times$ 3, 5Hz $\times$ 3  \\
\bottomrule
\end{tabular}
}
\caption{The granularity of 10 used in our HiP-AD model, including the three types of driving-style waypoints, represents fast, medium, and slow speeds with high and low frequency.}
\label{tab:supp_granularity}
\end{table}
